Cartesian Products Avoiding Patterns

The pattern avoidance problem seeks to construct a set with large fractal dimension that avoids a prescribed pattern, such as three term arithmetic progressions, or more general patterns, such as finding a set whose Cartesian product avoids the zero set of a given function. Previous work on the subject has considered patterns described by polynomials, or functions satisfying certain regularity conditions. We provide an exposition of some results in this setting, as well as considering new strategies to avoid what we call `rough patterns'. This thesis contains an expanded description of a method described in a previous paper by the author and his collaborators Malabika Pramanik and Joshua Zahl, as well as new results in the rough pattern avoidance setting. There are several problems that fit into the pattern of rough pattern avoidance. For instance, we prove that for any set $X$ with lower Minkowski dimension $s$, there exists a set $Y$ with Hausdorff dimension $1-s$ such that for any rational numbers $a_1, \dots, a_N$, the set $a_1 Y + \dots + a_N Y$ is disjoint from $X$, or intersects with $X$ solely at the origin. As a second application, we construct subsets of Lipschitz curves with dimension $1/2$ not containing the vertices of any isosceles triangle.

==> fourierDimension.tex <==
%% The following is a directive for TeXShop to indicate the main file
%%!TEX root = diss.tex

\chapter{Fourier Dimension and Fractal Avoidance}
\label{ch:FourierDimension}

There is much interplay between geometric measure theory and Fourier analysis. In particular, the Frostman dimension of a measure $\mu$ can be related to a integrability condition on it's Fourier transform. If we replace this integrability condition with a uniform bound on the decay of the Fourier transform, we obtain a stricter requirement. This leads to the \emph{Fourier dimension} of a measure. A natural question then arises; do sets supporting measures with large Fourier dimension naturally contain patterns?

\section{Basic Technique}

\begin{theorem}
	Let $K$ be a collection of at most $A \cdot N^s$, strongly non-diagonal sidelength $1/N$ dyadic cubes in $[0,1]^{nd}$. Then there exists a random set $X \subset [0,1]^d$, which is a union of sidelength $1/N$ dyadic cubes in $[0,1]^d$, and a constant $C$, depending only on $A$, $d$, and $n$, such that with probability $1 - C/\log N$,
	%
	\begin{itemize}
		\item $X^d \cap K = \emptyset$,
		\item If $\mu$ is the probability measure equal to a constant multiple of the Lebesgue measure on $X$, and supported on $X$, then for any $m \in \{ -N, \dots, N \}^d$,
		%
		\[ |\widehat{\mu}(m) - \widehat{dx}(m)| \leq \frac{C (\log N)^{1 - 1/n}}{N^{d-s/n}}. \]
	\end{itemize}
\end{theorem}
\begin{proof}
	Fix $p = 1/(AN^s \log N)^{1/n}$. Let $\{ X_Q \}$ be a family of independant and identically distributed $\{ 0, 1 \}$ valued Bernoulli random variable, for each sidelength $1/N$ dyadic cube, such that $\mathbf{P}(X_Q = 1) = p$ for each $Q$, and define $X = \bigcup \{ Q : X_Q = 1 \}$. Then Chernoff's inequality implies there exists a universal constant $c$ such that if $S = \sum_Q X_Q$, then
	%
	\[ \mathbf{P} \left( S \geq (1/2)(N^d p) \right) \geq 1 - 2 e^{- c N^d p}. \]
	%
	Substituting in parameters, we conclude
	%
	\begin{equation} \label{fourierdim1} \mathbf{P} \left( S \geq \left[ 1/2 A^{1/n} (\log N)^{1/n} \right] \cdot N^{d - s/n} \right) \geq 1 - 2 \exp \left( \frac{-N^{d-s/n}}{A^{1/n} (\log N)^{1/n}} \right) \end{equation}
	%
	Thus $X$ is the union of a large number of cubes with high probability.

	Given any cube $Q_1 \times \dots \times Q_n \in K$, we have
	%
	\[ \mathbf{P}(Q_1 \times \dots Q_n \subset X) = \mathbf{P}(Q_1 \in X, \dots, Q_n \in X) = p^n. \]
	%
	Thus
	%
	\[ \mathbf{E}(\# \{ Q_1 \times \dots \times Q_n \in X^n \}) \leq A N^s p^n = 1/\log N. \]
	%
	In particular, Markov's inequality implies
	%
	\begin{equation} \label{fourierdim2}
	\begin{split}
		\mathbf{P}(\# \{ Q_1 \times \dots \times Q_n \in X^n \} = 0) &= \mathbf{P}(\# \{ Q_1 \times \dots \times Q_n \in X^n \} < 1)\\
		&\geq 1 - 1/\log N.
	\end{split}
	\end{equation}
	%
	Thus $X^d$ avoids $K$ completely with high probability.

	Now we analyze the Fourier decay of the set $X$, conditioning on the value of $S$. For each cube $Q$, define
	%
	\[ f_Q = \begin{cases} \left( \frac{N^d}{S} - 1 \right) \cdot \mathbf{I}_Q & : X_Q = 1, \\ \left( -1 \right) \cdot \mathbf{I}_Q & : X_Q = 0. \end{cases} \]
	%
	If $f = \sum_Q f_Q$, then $f dx = d\mu - dx$. For each $x$, $\mathbf{E}[f_Q(x)|S] = 0$. If $x \not \in Q$, this is obvious, since $f_Q(x) = 0$ always holds, and if $x \in Q$, we find
	%
	\begin{align*}
		\mathbf{E}[f_Q(x)|S] &= \mathbf{P}(X_Q = 1|S) (N^d/S - 1) + \mathbf{P}(X_Q = 0|S) (-1)\\
		&= (S/N^d)(N^d/S - 1) + (1 - S/N^d)(-1) = 0,
	\end{align*}
	%
	This implies that for each $m \in \mathbf{Z}^d$,
	%
	\[ \mathbf{E} \left[ \widehat{f_Q}(m)|S \right] = \int \mathbf{E}[f_Q(x) | S] e^{- 2 \pi i x \cdot m}\; dx = 0. \]
	%
	Now $|\widehat{f_Q}(m)| \leq 1/S$ for all $Q$, and since the family $\big\{ \widehat{f_Q}(m) \big\}$ are independent random variables as $Q$ varies over all dyadic cubes, we can apply Hoeffding's inequality to conclude that there exists a universal constant $c$ such that for the random variable $\widehat{f}(m) = \sum \widehat{f_Q}(m)$,
	%
	\[ \mathbf{P} \left( |\widehat{f}(m)| \geq \log N /S \right) \leq 2/N^{c \log N} \]
	%
	If we now take a union bound over all $m \in \{ -N, \dots, N \}^d$, we can guarantee that
	%
	\begin{equation} \label{fourierdim3}
		\mathbf{P} \left( |\widehat{f}(m)| \leq \log N/S\ \text{for all $m \in \{ -N, \dots, N\}^d$} \right) \geq 1 - 2^{d+1}/N^{c \log N - d}.
	\end{equation}
	%
	Thus $\widehat{f}$ has good decay with high probability.

	Combining \eqref{fourierdim1}, \eqref{fourierdim2}, and \eqref{fourierdim3}, we conclude that there exists a constant $C$ such that with probability at least
	%
	\[ 1 - 2 \exp \left( \frac{-N^{d-s/n}}{A^{1/n} (\log N)^{1/n}} \right) - 1/\log N - \frac{2^{d+1}}{N^{c \log N - d}} \geq 1 - C / \log N, \]
	%
	the set $X$ avoids $K$, and for all $m \in \{ -N, \dots, N \}^d$,
	%
	\[ |\widehat{f}(m)| \leq \frac{C (\log N)^{1-1/n}}{N^{d-s/n}}. \qedhere \]
\end{proof}

\section{Another Try}

In the last few chapters, we have discovered that the presence of many configurations is not guaranteed by large Hausdorff dimension. We now turn to an analysis of a different dimensional quantity which in many cases gives much more structure than Hausdorff dimension. We construct a set $E$

\begin{proof}
	Let $S_0 = \{ 0 \}$. Then, given $S_k$, let $N^s$
	%
	\[ S_{k+1} = \left\{ (j, mN_{k+1}^{1-\alpha} + X_{jk}) : j \in S_k, 0 \leq m < N_{k+1}^\alpha \right\} \]
	% N_k = M_k^{1/\alpha}
	where $X_{jk}$ is chosen uniformly randomly from all integers in $[0,N_k^\alpha)$. Write $E_k = \{ \bigcup Q_j : j \in S_k \}$. Then $\#(S_{k+1}) = N_{k+1}^\alpha \#(S_k)$, and since $\#(S_0) = 1$, we find $\#(S_k) = (N_1 \dots N_k)^\alpha$. Now define $E_k = \{ \bigcup Q_j : j \in S_k \}$, and probability measures
	%
	\[ f_k = (N_1 \dots N_k)^{1 - \alpha} \mathbf{I}_{E_k}. \]
	%
	Then $\widehat{f_{k+1}}(m) - \widehat{f_k}(m) = \sum_{j \in S_k} Y_j(m)$, where
	%
	\[ Y_j(m) = \int_{I_j} (f_{k+1}(x) - f_k(x)) e(mx)\; dx \]
	%
	Note that $\mathbf{E}[f_{k+1}(x)] = \mathbf{E}[f_k(x)]$ for each $x$, so that $\mathbf{E}[Y_j(m)] = 0$. Note also that
	%
	\[ |Y_j(m)| \leq 2l_k / l_{k+1}^{1-\alpha} = \frac{2 N_{k+1}^{1-\alpha}}{(N_1 \dots N_k)^\alpha}. \]
	%
	Thus Hoeffding's inequality implies
	%
	\begin{align*}
		\mathbf{P} \left( |\widehat{f_{k+1}}(m) - \widehat{f_k}(m)| \geq t \right) &\leq 4 \exp \left( - \left( t \frac{(N_1 \dots N_k)^\alpha}{4 N_{k+1}^{1-\alpha} \#(S_k)^{1/2}} \right)^2 \right)\\
		&\leq 4 \exp \left( - \left( t \frac{(N_1 \dots N_k)^{\alpha/2}}{2 N_{k+1}^{1-\alpha}} \right)^2 \right)
	\end{align*}
	%
	Thus we can guarantee with high probability that for all $m$,
	%
	\[ |\widehat{f_{k+1}}(m) - \widehat{f_k}(m)| \lessapprox \frac{N_{k+1}^{1-\alpha}}{(N_1 \dots N_k)^{\alpha/2}} \]
	%
	So if $N_{k+1} \lesssim (N_1 \dots N_k)^\varepsilon$ for all $\varepsilon > 0$, we obtain the right bound. But we need something deeper.

	Take 2: Write
	%
	\[ f_{k+1}(x) = (N_1 \dots N_{k+1})^{1-\alpha} \sum_{j \in S_k} \sum_{m = 0}^{N_{k+1}^{1-\alpha}} Y_{jm} \]
	%
	where $Y_{jm}$ is the indicator function of
	%
	\[ \left[ \frac{j}{N_1 \dots N_k} + \frac{m}{N_1 \dots N_{k+1}^\alpha} + \frac{X_{jk}}{N_1 \dots N_{k+1}}, \frac{j}{N_1 \dots N_k} + \frac{m}{N_1 \dots N_{k+1}^\alpha} + \frac{X_{jk} + 1}{N_1 \dots N_{k+1}} \right] \]
	%
	Note that
	%
	\[ \widehat{Y_{jm}}(n) = \frac{1}{2 \pi i n} e \left( \frac{j n}{N_1 \dots N_k} + \frac{m n}{N_1 \dots N_{k+1}^\alpha} + \frac{X_{jk} n}{N_1 \dots N_{k+1}} \right) \left( e \left( \frac{n}{N_1 \dots N_{k+1}} \right) - 1 \right), \]
	%
	and
	%
	\begin{align*}
		\mathbf{E} \left(\widehat{Y_{jm}}(n) \right) &= \frac{1}{2 \pi i n N_{k+1}^\alpha} e \left( \frac{jn}{N_1 \dots N_k} + \frac{mn}{N_1 \dots N_{k+1}^\alpha} \right) \left( e \left( \frac{ N_{k+1}^\alpha n}{N_1 \dots N_{k+1}} \right) - 1 \right).
	\end{align*}
	%
	and $|\widehat{Y_{jm}}| \leq 1/(N_1 \dots N_{k+1})$. Thus Hoeffding's inequality implies, if we ignore the expectation,
	%
	%
	\begin{align*}
		\mathbf{P} \left( |\widehat{f_{k+1}}(n)| \geq t (N_1 \dots N_{k+1})^{1-\alpha} \right) &\leq 4 \exp \left( \frac{-t^2 (N_1 \dots N_{k+1})^2}{4(N_1 \dots N_{k+1})^\alpha} \right)\\
		&\leq 4 \exp \left( - \left( t (N_1 \dots N_{k+1})^{1 - \alpha/2} / 2 \right)^2 \right).
	\end{align*}
	%
	Thus with high probability, for all $|n| \leq N_1 \dots N_{k+1}$,
	%
	\[ |\widehat{f_{k+1}}(n)| \lessapprox \frac{1}{(N_1 \dots N_{k+1})^{\alpha/2}}. \]
\end{proof}




\section{Schmerkin's Method}

We now try and adapt Schmerkin's Method to our situation, introducing translations into the avoiding set. Let $K \subset \mathbf{Z}_N^n$. Our goal is to find $X \subset \mathbf{Z}_N$ such that if $x_1, \dots, x_n$ are distinct, then $(x_1, \dots, x_n) \not \in K$, such that if $f: \mathbf{Z}_N \to \mathbf{R}$ is the probability distribution which uniformly randomly chooses a point on $X$, such that the Fourier transform of $f$ has small $L^\infty$ norm.

We consider an intermediary scale $M$, with $M \divides N$. Then we consider the set
%
\[ K' = \{ x \in \mathbf{Z}_N^n : \text{There is $y \in K$ with $x - y \in M \mathbf{Z}_N^n$} \}. \]
%
We construct $X$ such that if $x_1, \dots, x_n \in X$ are distinct, then $(x_1, \dots, x_n) \not \in Y$. In particular, this means that if we define, for each $x \in X$, a uniformly random selected integer $n_x \in M \mathbf{Z}_N$, then we can define $x' = x + n_x$, and $X' = \{ x' : x \in X \}$. Now if $I_x: \mathbf{Z}_N \to \mathbf{R}$ denotes the delta function at $x'$, then
%
\[ \widehat{I_x}(k) = (1/N) e(-kx'/N) = (1/N) e(-kx/N) e(-n_x). \]
%
And so
%
\begin{align*}
	\mathbf{E}(\widehat{I_x}(k)) &= (M/N) e(-kx/N) \sum_{m = 1}^{N/M} e(-(kM/N)m).
\end{align*}
%
If $kM/N \not \in \mathbf{Z}$, $\mathbf{E}(\widehat{I_x}(k)) = 0$. If $kM/N \in \mathbf{Z}$, then $\mathbf{E}(\widehat{I_x}(k)) = e(-kx/N)$. And
%
\[ |\widehat{I_x}(k)| \leq 1. \]
%
Since $I_x$ is independant, we can apply Hoeffding's inequality to conclude that
%
\[ \mathbf{P} \left( \widehat{f}(k) \geq t \right) \leq \exp \left( \frac{-t^2}{4|X|} \right) \]
%
so $\widehat{f}(k) \lesssim |X|^{1/2}$ with high probability. This should give the Fourier dimension bound we want? Except we do lose some dimension by introducing the parameter $M$. If we pick $N$ to be very large, but $M$ very small, then this shouldn't introduce many problems? What about if we pick $M$ randomly to prevent problems on the linear frequencies?






\section{Tail Bounds on Cube Selection}

The aim of this section is to obtain tail bounds on the total number of intersections between the random set we select in the discrete selection schema, with the goal of obtaining a Fourier dimension bound on the set we construct. Consider the random process generating our interval selection scheme. We have three fixed lengths $l$, $r$, and $s$. We start with a set $E$, which is a non-empty union of cubes in $\B^d_l$, and a set $G$, which is a union of cubes in $\B^{dn}_s$. For each cube $J \in \B^d_r(E)$, we select a single random element of $\B^d_s(J)$, denoted $J_I$. We let $U = \bigcup J_I$. The aim of this section is to obtain tail bounds on the size of the random set
%
\[ \mathcal{K}(U) = \{ K \in \B^{dn}_s(G): K \in U^n, K\ \text{strongly non-diagonal} \}. \]
%
Here, this is obtained by applying the statistical decoupling techniques of Bourgain and Tzafriri.

To understand the distribution of this random variable, it will be convenient to simplify notation. We write $\mathbf{I}(I_J = I_0)$ as $X_{J,I_0}$. We then set
%
\[ Z = \# \mathcal{K}(U) = \sum_{J_1, \dots, J_n} \sum_K \left( \prod_{i = 1}^n X_{J_i,K_i} \right), \]
%
where $J_1, \dots, J_n$ ranges over all distinct choices of $n$ elements from $\B^d_l(E)$, and $K = K_1 \times \dots \times K_n$ ranges over all elements of $\B^{dn}_l(G) \cap \B^{dn}_s(J_1 \times \dots \times J_n)$. The random cubes $\{ I_J \}$ form an independant family, which should make the distribution easier to bound. But $Z$ is a multiplicative linear combination of this independant family. Random variables of this form as known as a \emph{chaos}.

The idea behind statistical decoupling is to obtain tail bounds on the chaos $Z$ by studying the tail bounds on the modified random variable
%
\[ W = \sum_{J_1, \dots, J_n} \sum_K \left( \prod_{i = 1}^n X_{J_i,K_i}^i \right), \]
%
where $X^1, \dots, X^n$ are independant and identically distributed copies of $X$.

\begin{lemma} \label{decouplinglemma}
	Let $F: [0,\infty) \to [0,\infty)$ be a monotone, convex function. Then
	%
	\[ \EE(F(Z)) \leq \EE(F(n^n W)). \]
\end{lemma}
\begin{proof}
	Consider a partition $\mathcal{J}_1, \dots, \mathcal{J}_n$ selected at random from all possible partitions of $\B^d_s(E)$ into $n$ classes. Then, for any distinct set of intervals $J_1, \dots, J_n \in \B^d_s(E)$,
	%
	\begin{equation} \label{partitionprob}
		\PP(J_1 \in \mathcal{J}_1, \dots, J_n \in \mathcal{J}_n) = \PP(J_1 \in \mathcal{J}_1) \dots \PP(J_n \in \mathcal{J}_n) = 1/n^n.
	\end{equation}
	%
	Thus if we consider
	%
	\[ Z' = \sum_{J_1 \in \mathcal{J}_1, \dots, J_n \in \mathcal{J}_n} \sum_K \left( \prod_{i = 1}^n X_{J_i,K_i} \right), \]
	%
	where $J_i$ ranges over elements of $\mathcal{J}_i$ for each $i \in [n]$. If we let $\EE_{\mathcal{J}}$ denote conditioning with respect to all random variables except those depending on $\mathcal{J}_1, \dots, \mathcal{J}_n$, then \eqref{partitionprob} implies
	%
	\begin{align*}
		\EE_{\mathcal{J}}(Z') &= \sum_{J_1, \dots, J_n} \sum_K \PP(J_1 \in \mathcal{J}_1, \dots, J_n \in \mathcal{J}_n) \left( \prod_{i = 1}^n X_{J_i,K_i} \right) = Z/n^n.
	\end{align*}
	%
	Thus Jensen's inequality implies that
	%
	\[ F(Z) = F(n^n \EE_{\mathcal{J}}(Z')) \leq \EE_{\mathcal{J}} F(n^n Z'). \]
	%
	In particular, this means we can select a single, non-random partition $\mathcal{J}_1, \dots, \mathcal{J}_n$ of $\B^d_s(E)$ such that $F(Z) \leq F(n^n Z')$. Because $\mathcal{J}_1, \dots, \mathcal{J}_n$ are disjoint sets, $Z'$ is identically distributed to
	%
	\[ W' = \sum_{J_1 \in \mathcal{J}_1, \dots, J_n \in \mathcal{J}_n} \sum_K \left( \prod_{i = 1}^n X_{J_i,K_i}^i \right). \]
	%
	But $W' \leq W$, and so by monotonicity,
	%
	\[ \EE(F(Z)) \leq \EE(F(n^n W')) \leq \EE(F(n^n W)). \qedhere \]
\end{proof}

\begin{lemma}
	MOMENT BOUND THEOREM.
\end{lemma}
\begin{proof}
	We now bound the moments of $W$, which by Lemma \ref{decouplinglemma} bounds the moments of $Z$. We write
	%
	\[ W^m = \sum_{J_{j,i}} \sum_{K_1, \dots, K_m} \left( \prod_{i = 1}^n \prod_{j = 1}^m X_{J_{j,i}, K_{j,i}}^i \right). \]
	%
	Thus
	%
	\[ \EE(W^m) = \sum_{J_{j,i}} \sum_{K_1, \dots, K_m} \prod_{i = 1}^n \EE \left( \prod_{j = 1}^m X_{J_{j,i}, K_{j,i}}^i \right) \]
	%
	The inner expectation is zero except if $\pi(K_{j,i}) = J_{j,i}$ for all $j$ and $i$, and also, if $\pi(K_{j_0,i}) = \pi(K_{j_1,i})$, then $K_{j_0,i} = K_{j_1,i}$. And then the expectation is $\varepsilon^{\# \{ K_{1,i}, \dots, K_{m,i} \}}$.
\end{proof}

\section{Singular Value Decomposition of Tensors}

An \emph{$n$ tensor} with respect to $\RR^{k_1}, \dots, \RR^{k_n}$, is a multi-linear function
%
\[ A: \RR^{k_1} \times \dots \times \RR^{k_n} \to \RR. \]
%
The family of all $n$ tensors forms a vector space, denoted $\RR^{k_1} \otimes \dots \otimes \RR^{k_n}$, or $\bigotimes \RR^{k_i}$. Given a family of vectors $v_i$, with $v_i \in \RR^{k_i}$, we can consider a tensor $v_1 \otimes \dots \otimes v_n$, such that
%
\[ (v_1 \otimes \dots \otimes v_n)(w_1, \dots, w_n) = (v_1 \cdot w_1) \dots (v_n \cdot w_n). \]
%
It is easily verified that a basis for $\RR^{k_1} \otimes \dots \otimes \RR^{k_n}$ is given by
%
\[ \{ e_{j_1} \otimes \dots \otimes e_{j_n} : j_i \in [k_i] \}. \]
%
Thus a tensor $A$ can be identified with a family of coefficients
%
\[ \{ A_{j_1 \dots j_n} : 1 \leq j_i \leq k_i \} \]
%
such that
%
\[ A(v_1,\dots,v_n) = \sum A_{j_1 \dots j_n} \cdot e_{j_1} \otimes \dots \otimes e_{j_n}. \]
%
From this perspective, a tensor is a multi-dimensional array given by $n$ indices. This basis induces a natural inner product for which the basis is orthonormal. The norm with respect to this inner product is called the \emph{Frobenius norm}, denoted $\| A \|_F$.

Recall that if $A$ is a rank $r$, $m \times n$ matrix, then the \emph{singular value decomposition} says that there are orthonormal families of vectors $\{ u_1, \dots, u_r \}$ and $\{ v_1, \dots, v_r \}$ in $\RR^m$ and $\RR^n$ respectively, and values $s_1, \dots, s_r > 0$ such that $A = \sum s_i (u_i^T v_i)$. We may view $A$ as a 2 tensor in $\RR^m \otimes \RR^n$ by setting $A(v,w) = v^T A w$. Then the singular value decomposition says that $A = \sum s_i (u_i \otimes v_i)$. Thus, viewing $A$ as a bilinear function, for any vectors $x \in \RR^m$ and $y$ in $\RR^n$, $A(x,y) = \sum s_i (u_i \cdot x) (v_i \cdot y)$. We want to try and generalize this result to $n$ tensors in $\RR^{k_1} \otimes \dots \otimes \RR^{k_n}$.

One can reduce certain quantities over tensors to quantities defined with respect to linear maps. For instance, for each index $i_0 \in [n]$, we can define a linear map
%
\[ A_i: \bigotimes_{i' \neq i} \RR^{k_{i'}} \to \RR^{k_i} \]
%
by letting $A_{i_0}(v_1, \dots, \widehat{v_i}, \dots, v_n)$ to be the unique vector $w \in \RR^{k_i}$ such that for any vector $v_i \in \RR^{k_i}$,
%
\[ v_i \cdot w = A(v_1, \dots, v_n). \]
%
The matrix $A_i$ is known as the \emph{$i$'th unfolding of $A$}. We define the $i$ rank of $A$ to be $\text{rank}_i(A) = \text{rank}(A_i)$. This generalizes the column and row rank of matrices. Unlike in the case of matrices, these quantities can differ for different indices $i$. One can also obtain the $i$ rank

The natural definition of the rank of a tensor in the study of the higher order singular value decomposition is defined in analogy with the fact that a rank $r$ matrix can be written as the sum of $r$ rank one matrices. We say a tensor is rank one if it can be written in the form $v_1 \otimes \dots \otimes v_n$ for some vectors $v_i \in \RR^{k_i}$. The \emph{rank} of a tensor $A$, denoted $\text{rank}(A)$, is the minimal number of rank one tensors which can be written in a linear combination to form $A$. We have $\text{rank}(A_i) \leq \text{rank}(A)$ for each $i$, but there may be a gap in these ranks.

To obtain an SVD decomposition, fix an index $i$. Then we can perform a singular value decomposition on $A_i$, obtaining orthonormal basis

\section{Decoupling Concentration Bounds}

We require some methods in non-asymptotic probability theory in order to understand the concentration structure of the random quantities we study. Most novel of these is relying on a probabilistic decoupling bound of Bourgain.

In this section, we fix a single underlying probability space, assumed large enough for us to produce any additional random quantities used in this section. Given a scalar valued random variable $X$, we define its \emph{Orlicz norm} as
%
\[ \| X \|_{\psi_2} = \inf \left\{ \lambda \geq 0 : \EE \left(\exp \left( |X|^2/\lambda^2 \right) \right) \leq 2 \right\}. \]
%
The family of random variables with finite Orlicz norm forms a Banach space, known as the space of \emph{subgaussian random variables}.

\begin{theorem}
	Let $X$ be a sub-gaussian random variable.
	%
	\begin{itemize}
		\item For all $t \geq 0$,
		%
		\[ \PP \left( |X| \geq t \right) \leq 2 \exp \left( \frac{-t^2}{\| X \|_{\psi_2}^2} \right). \]

		\item Conversely, if there is a constant $K > 0$ such that for all $t \geq 0$,
		%
		\[ \PP \left( |X| \geq t \right) \leq 2 \exp \left( \frac{-t^2}{K^2} \right), \]
		%
		then $\| X \|_{\psi_2} \leq 2K$.

		\item For any bounded random variable $X$, $\| X \|_{\psi_2} \lesssim \| X \|_\infty$.

		\item $\| X - \EE X \|_{\psi_2} \lesssim \| X \|$.

		\item If $X_1, \dots, X_n$ are independent, then
		%
		\[ \| X_1 + \dots + X_n \|_{\psi_2} \lesssim \left( \| X_1 \|_{\psi_2}^2 + \dots + \| X_n \|_{\psi_2}^2 \right)^{1/2}. \] 
	\end{itemize}
\end{theorem}
\begin{proof} See \cite{Vershynin}. \end{proof}

Given a random vector $X$, taking values in $\RR^n$, we say it is \emph{uniformly subgaussian} if there is a constant $A$ such that for any $x \in \RR^n$, $\| X \cdot x \|_{\psi_2} \leq A \cdot |x|$. We define
%
\[ \| X \|_{\psi_2} = \sup_{|x| = 1} \| X \cdot x \|_{\psi_2}, \]
%
so that $\| X \cdot x \|_{\psi_2} \leq \| X \|_{\psi_2} \cdot |x|$ for any random vector $X$.

The classic Hanson-Wright inequality gives a concentration bound for the magnitude of a quadratic form $X^T A X$ in terms of the matrix norms of $A$, assuming $X$ is a random vector with independant, mean zero, subgaussian coordinates.

\begin{theorem}[Hanson-Wright]
	Let $X = (X_1, \dots, X_k)$ be a random vector with independant, mean zero, subgaussian coordinates, with $\| X_i \|_{\psi_2} \leq K$ for each $i$, and let $A$ be a diagonal-free $k \times k$ matrix. Then there is a universal constant $c$ such that for every $t \geq 0$,
	%
	\[ \PP \left( |X^TAX| \geq t \right) \leq 2 \exp \left( -c \cdot \min \left( \frac{t^2}{K^4 \| A \|_F^2}, \frac{t}{K^2 \| A \|} \right) \right). \]
	%
	Here $\| A \|$ is the operator norm of $A$, and $\| A \|_F$ it's Frobenius norm.
\end{theorem}

In our work, we require a modified version of the Hanson Wright inequality where we replace the independant random variables $X_1, \dots, X_k$ with independant random vectors taking values in $\RR^d$, and where $A$ is replaced with a $n$ tensor on $\RR^{k \times d}$. To make things more tractable, we assume that $A_I = 0$ for each multi-index $I = ((i_1,j_1), \dots, (i_n,j_n))$ if there is $r \neq r'$ with $i_r = i_{r'}$. If this is satisfied, we say $A$ is a \emph{non-diagonal tensor}.

\begin{theorem}
	Let $X = (X_1, \dots, X_k)$, where $X_1, \dots, X_k$ are independant, mean zero random vectors taking values in $\RR^d$, with $\| X_i \|_{\psi_2} \leq K$ for each $i$. Let $A$ be a non-diagonal $n$-tensor in $\RR^{k \times d}$. Then for $t \geq 0$,
	%
	\[ \PP \left( |A(X,\dots,X)| \geq t \right) \leq 2 \cdot \exp \left( - c(n) \cdot \min \left( \frac{t^2}{K^4 \| A \|_F^2}, \dots, \frac{t^{2/n}}{K^{4/n} \| A \|_F^{2/n}} \right) \right). \]
\end{theorem}

The main technique involved is a statistical decoupling result due to J. Bourgain and L. Tzafriri. We follow the proof of the Hanson-Wright inequality from \cite{Vershynin}, altering various calculations to incorporate the vector-valued coordinates $X_1, \dots, X_n$, and incorporating more robust calculations of the moments of higher order Gaussian chaos.

\begin{lemma}[Decoupling]
	If $F: \RR \to \RR$ is convex, and $X = (X_1, \dots, X_k)$, where $X_1, \dots, X_k$ are independant, mean zero random vectors taking values in $\RR^d$. If $A$ is a non-diagonal $n$-tensor in $\RR^{d \times k}$, then
	%
	\[ \EE(F(A(X,\dots,X))) \leq \EE(F(n^n \cdot A(X^1,X^2,\dots,X^n))), \]
	%
	where $X^1, \dots, X^n$ are independant copies of $X$.
\end{lemma}
\begin{proof}
	Given a set $I \subset [k]$, let $\pi_I: \RR^{k \times d} \to \RR^{k \times d}$ be defined by
	%
	\[ \pi_{I}(X)_{ij} = \begin{cases} X_{ij} &: \text{if}\ i \in I, \\ 0 &: \text{if}\ i \not \in I \end{cases}. \]
	%
	Thus given $X = (X_1, \dots, X_k)$, the vector $\pi_I(X)$ is obtained by zeroeing out all vectors $X_i$ with $i \not \in I$. Consider a random partition of $[k]$ into $n$ classes $I_1, \dots, I_n$, chosen uniformly at random. Thus given any $x \in \RR^{d \times k}$, we have
	%
	\[ \EE(A(\pi_{I_1}(x),\dots,\pi_{I_n}(x))) = \sum_{I=((i_1,j_1),\dots,(i_n,j_n))} A_I \cdot x_{i_1 j_1} \dots x_{i_n j_n} \PP(i_1 \in I_1, \dots, i_n \in I_n). \]
	%
	If $A_I \neq 0$, the indices $\{ i_r \}$ are distinct from one another. Since $(I_1,\dots,I_n)$ is selected uniformly at random, this means the positions of the indices $i_r$ are independent of one another. Thus
	%
	\[ \PP(i_1 \in I_1, \dots, i_n \in I_n) = \PP(i_1 \in I_1) \dots \PP(i_n \in I_n) = 1/n^n. \]
	%
	Thus we have shown
	%
	\[ A(x,\dots,x) = n^n \cdot \EE(A(\pi_{I_1}(x), \dots, \pi_{I_n}(x))). \]
	%
	In particular, substituting $X$ for $x$, we have
	%
	\[ A(X,\dots,X) = n^n \cdot \EE_I(A(\pi_{I_1}(X), \dots, \pi_{I_n}(X))) \]
	%
	Applying Jensen's inequality, we find
	%
	\begin{align*}
		\EE_X(F(A(X,\dots,X))) &= \EE_X(F(n^n \cdot \EE_I(A(\pi_{I_1}(X), \dots, \pi_{I_n}(X)))))\\
		&\leq \EE_X \EE_I F(n^n \cdot A(\pi_{I_1}(X), \dots, \pi_{I_n}(X)))\\
		&= \EE_I \EE_X F(n^n \cdot A(\pi_{I_1}(X), \dots, \pi_{I_n}(X))).
	\end{align*}
	%
	Thus we may select a \emph{deterministic} partition $I$ for which
	%
	\[ \EE(F(A(X,\dots,X))) \leq \EE(F(n^n \cdot A(\pi_{I_1}(X),\dots,\pi_{I_n}(X)))). \]
	%
	Since the classes $I_1, \dots, I_n$ are disjoint from one another, $(\pi_{I_1}(X), \dots, \pi_{I_n}(X))$ is identically distributed to $(\pi_{I_1}(X^1), \dots, \pi_{I_n}(X^n))$, so
	%
	\[ \EE(F(n^n \cdot A(\pi_{I_1}(X),\dots,\pi_{I_n}(X)))) = \EE(F(n^n \cdot A(\pi_{I_1}(X^1),\dots,\pi_{I_n}(X^n)))). \]
	%
	Let $Z = A(X^1,\dots,X^n) - A(\pi_{I_1}(X^1),\dots,\pi_{I_n}(X^n))$. If $\EE'$ denotes conditioning with respect to $\pi_{I_1}(X^1), \dots, \pi_{I_n}(X^n)$, then this expectation fixes $A(\pi_{I_1}(X_1),\dots,\pi_{I_n}(X_n))$, but $\EE'(Z) = 0$. Thus we can apply Jensen's inequality again to conclude
	%
	\begin{align*}
		\EE(F(n^n \cdot A(\pi_{I_1}(X^1),\dots,\pi_{I_n}(X^n)))) &= \EE(F(n^n \cdot \EE'(A(\pi_{I_1}(X^1), \dots, \pi_{I_n}(X^n)) + Z)))\\
		&= \EE(F(n^n \cdot \EE'(A(X^1,\dots,X^n))))\\
		&\leq \EE(\EE'(F(n^n A(X^1,\dots,X^n))))\\
		&= \EE(F(n^n A(X^1,\dots,X^n))). \qedhere
	\end{align*}
\end{proof}

\begin{remark}
	Note this theorem also implies that for each $\lambda \in \RR$,
	%
	\[ \EE(F((\lambda/n^n) \cdot A(X,\dots,X))) \leq \EE(F(\lambda \cdot A(X^1,\dots,X^n))). \]
\end{remark}

\begin{lemma}[Comparison]
	Let $X^1,\dots,X^n$ be independant random vectors taking values in $\RR^{k \times d}$
\end{lemma}

To make things easy for ourselves, we assume that $A$ vanishes along it's diagonal. Reinterpreting the quantities in the Hanson-Wright inequality in this setting gives the result. For each $i$ and $j$, we define $A_{ij}$ be an $d \times d$ matrix, then we set $X^T A X = \sum X_i^T A_{ij} X_j$,
%
\[ \| A \|_F = \sqrt{\sum \| A_{ij} \|_F^2}, \quad\text{and}\quad \| A \| = \sup \left\{ |\sum x_i^T A_{ij} y_j| : \sum |x_i|^2 = \sum |y_j|^2 = 1 \right\}. \]
%
These are precisely the definitions of the operator norm and Frobenius norm if we interpret $A$ as a $dn \times dn$ matrix by expanding out the entries of each $A_{ij}$, and $X$ as a random vector taking values in $\RR^{dn}$ by expanding out the entries of each $X_i$.

\endinput

==> glossary.tex <==
%% The following is a directive for TeXShop to indicate the main file
%%!TEX root = diss.tex

\chapter{Glossary}

This glossary uses the handy \latexpackage{acroynym} package to automatically
maintain the glossary.  It uses the package's \texttt{printonlyused}
option to include only those acronyms explicitly referenced in the
\LaTeX\ source.

% use \acrodef to define an acronym, but no listing
\acrodef{UI}{user interface}
\acrodef{UBC}{University of British Columbia}

% The acronym environment will typeset only those acronyms that were
% *actually used* in the course of the document
\begin{acronym}[ANOVA]
\acro{ANOVA}[ANOVA]{Analysis of Variance\acroextra{, a set of
  statistical techniques to identify sources of variability between groups}}
\acro{API}{application programming interface}
\acro{CTAN}{\acroextra{The }Common \TeX\ Archive Network}
\acro{DOI}{Document Object Identifier\acroextra{ (see
    \url{http://doi.org})}}
\acro{GPS}[GPS]{Graduate and Postdoctoral Studies}
\acro{PDF}{Portable Document Format}
\acro{RCS}[RCS]{Revision control system\acroextra{, a software
    tool for tracking changes to a set of files}}
\acro{TLX}[TLX]{Task Load Index\acroextra{, an instrument for gauging
  the subjective mental workload experienced by a human in performing
  a task}}
\acro{UML}{Unified Modelling Language\acroextra{, a visual language
    for modelling the structure of software artefacts}}
\acro{URL}{Unique Resource Locator\acroextra{, used to describe a
    means for obtaining some resource on the world wide web}}
\acro{W3C}[W3C]{\acroextra{the }World Wide Web Consortium\acroextra{,
    the standards body for web technologies}}
\acro{XML}{Extensible Markup Language}
\end{acronym}

% You can also use \newacro{}{} to only define acronyms
% but without explictly creating a glossary
% 
% \newacro{ANOVA}[ANOVA]{Analysis of Variance\acroextra{, a set of
%   statistical techniques to identify sources of variability between groups.}}
% \newacro{API}[API]{application programming interface}
% \newacro{GOMS}[GOMS]{Goals, Operators, Methods, and Selection\acroextra{,
%   a framework for usability analysis.}}
% \newacro{TLX}[TLX]{Task Load Index\acroextra{, an instrument for gauging
%   the subjective mental workload experienced by a human in performing
%   a task.}}
% \newacro{UI}[UI]{user interface}
% \newacro{UML}[UML]{Unified Modelling Language}
% \newacro{W3C}[W3C]{World Wide Web Consortium}
% \newacro{XML}[XML]{Extensible Markup Language}


==> lowrank.tex <==
%% The following is a directive for TeXShop to indicate the main file
%%!TEX root = diss.tex

\chapter{Extensions to Low Rank Configurations}
\label{ch:LowRank}



\section{Boosting the Dimension of Pattern Avoiding Sets by Low Rank Coordinate Changes}

We now consider finding subsets of $[0,1]$ avoiding solutions to the equation $y = f(Tx)$, where $T$ is a rank $k$ linear transformation with integer coefficients with respect to standard coordinates, and $f$ is real-valued and Lipschitz continuous. Fix a constant $A$ bounding the operator norm of $T$, in the sense that $|Tx| \leq A|x|$ for all $x \in \mathbf{R}^n$, and a constant $B$ such that $|f(x+y) - f(x)| \leq B|y|$ for all $x$ and $y$ for which the equation makes sense (if $f$ is $C^1$, this is equivalent to a bound $\| \nabla f \|_\infty \leq B$). Consider sets $J_0, J_1, \dots, J_n, \subset [0,1]$, which are unions of intervals of length $1/M$, with startpoints lying on integer multiples of $1/M$. The next theorem works as a `building block lemma' used in our algorithm for constructing a set avoiding solutions to the equation with Hausdorff dimension $k$ and full Minkowski dimension.

\begin{theorem}
    For infinitely many integers $N$, there exists $S_i \subset J_i$ avoiding solutions to $y = f(Tx)$ with $y \in S_0$ and $x_n \in S_n$, such that
    %
    \begin{itemize}
        \item For $n \neq 0$, if we decompose each $J_i$ into length $1/N$ consecutive intervals, $S_i$ contains an initial portion $\Omega(1/N^k)$ of each length $1/N$ interval. This part of the decomposition gives the Hausdorff dimension $1/k$ bound for the set we will construct.

        \item If we decompose $J_i$ into length $1/N$ intervals, and then subdivide these intervals into length $\Omega(1/N^k)$ intervals, then $S_0$ contains a subcollection of these $1/N^k$ intervals which contains a total length $\Omega(1/N)$ of a fraction $1 - 1/M$ of the length $1/N$ intervals. This property gives that our resultant set will have full Minkowski dimension.
    \end{itemize}
    %
    The implicit constants in these bounds depend only on $A$, $B$, $n$, and $k$.
\end{theorem}
\begin{proof}
Split each interval of $J_a$ into length $1/N$ intervals, and then set
%
\[ \mathbf{A} = \{ x : x_a\ \text{is a startpoint of a $1/N$ interval in $J_a$} \} \]
%
Since the startpoints of the intervals are integer multiples of $1/N$, $T(\mathbf{A})$ is contained with a rank $k$ sublattice of $(\mathbf{Z}/N)^m$. The operator norm also guarantees $T(\mathbf{A})$ is contained within the ball $B_A$ of radius $A$ in $\mathbf{R}^m$. Because of the lattice structure of the image, $| x - y | \gtrsim_n 1/N$ for each distinct pair $x,y \in T(\mathbf{A})$. For any $R$, we can cover $\Sigma \cap B_A$ by $O_{n,k}((A/R)^k)$ balls of radius $R$. If $R \gtrsim_n 1/N$, then each ball can contain only a single element of $T(\mathbf{A})$, so we conclude that $|T(\mathbf{A})| \lesssim_{n,k} (AN)^k$. If we define the set of `bad points' to be
%
\[ \mathbf{B} = \{ y \in [0,1] : \text{there is $x \in \mathbf{A}$ such that $y = f(T(x))$} \} \]
%
Then
%
\[ |\mathbf{B}| = |f(T(\mathbf{A}))| \leq |T(\mathbf{A})| = O_{A,n,k}(N^k) \]
%
For simplicity, we now introduce an integer constant $C_0 = C_0(A,n,k,M)$ such that $|\mathbf{B}| \leq (C_0/M^2) N^k$. We now split each length $1/M$ interval in $J_0$ into length $1/N$ intervals, and filter out those intervals containing more than $C_0N^{k-1}$ elements of $\mathbf{B}$. Because of the cardinality bound we have on $\mathbf{B}$ there can be at most $N/M^2$ such intervals, so we discard at most a fraction $1/M$ of any particular length $1/M$ interval in $J_0$. If we now dissect the remaining intervals into $4C_0N^{k-1}$ intervals of length $1/4C_0N^k$, and discard any intervals containing an element of $\mathbf{B}$, or adjacent to such an interval, then the remaining such intervals $I$ satisfy $d(I,\mathbf{B}) \geq 1/4C_0N^k \gtrsim_{A,n,M,k}(1/N^k)$, and because of our bound on the number of elements of $\mathbf{B}$ in these intervals, there are at least $C_0N^{k-1}$ intervals remaining, with total length exceeding $C_0N^{k-1}/4C_0N^k = \Omega(1/N)$. If $f$ is $C^1$ with $\| \nabla f \|_\infty \leq B$, or more generally, if $f$ is Lipschitz continuous of magnitude $B$, then
%
\[ | f(Tx) - f(Tx')| \leq AB |x - x'| \]
%
and so we may choose $S_i \subset J_i$ by thickening each startpoint $x \in J_i$ to a length $O(1/N^k)$ interval while still avoiding solutions to the equation $y = f(T(x))$.
\end{proof}

\begin{remark}
    If $T$ is a rank $k$ linear transformation with rational coefficients, then there is some number $a$ such that $aT$ has integer coefficients, and then the equation $y = f(Tx)$ is the same as the equation $y = f_0((aT)(x))$, where $f_0(x) = f(x)/a$. Since $f_0$ is also Lipschitz continuous, we conclude that we still get the dimension $1/k$ bound if $T$ has rational rather than integral coefficients. More generally, this trick shows the result applies unperturbed if all coefficients of $T$ are integer multiples of some fixed real number. More generally, by varying the lengths of our length $1/N$ decomposition by a constant amount, we can further generalize this to the case where each column of $T$ are integers multiples of some fixed real number.
\end{remark}

\begin{remark}
    To form $\mathbf{A}$, we take startpoints lying at equal spaced $1/N$ points. However, by instead taking startpoints at varying points in the length $1/N$ intervals, we might be able to make points cluster more than in the original algorithm. Maybe the probabalistic method would be able to guarantee the existence of a choice of startpoints whose images are tightly clustered together.
\end{remark}

\begin{remark}
    Since the condition $y = f(Tx)$ automatically assumes a kind of `non-vanishing derivative' condition on our solutions, we do not need to assume the regularity of $f$, and so the theorem extends naturally to a more general class of functions than Rob's result, i.e. the Lipschitz continuous functions.
\end{remark}

Using essentially the same approach as the last argument shows that we can avoid solutions to $y = f(Tx)$, where $y$ and $x$ are now vectors in some $\mathbf{R}^m$, and $T$ has rank $k$. If we consider unions of $1/M$ cubes $J_0, \dots, J_n$. If we fix startpoints of each $x_k$ forming lattice spaced apart by $\Omega(1/N)$, and consider the space $\mathbf{A}$ of products, then there are $O(N^k)$ points in $T(\mathbf{A})$, and so there are $O(N^k)$ elements in $\mathbf{B}$. We now split each $1/M$ cube in $J_0$ into length $1/N$ cubes, and discard those cubes which contain more than $O(N^{k-m})$ bad points, then we discard at most $1 - 1/M$ of all such cubes. We can dissect the remaining length $1/N$ cubes into $O(N^{k-m})$ length $\Omega(1/N^{k/m})$ cubes, and as in the previous argument, the cubes not containing elements of $\mathbf{B}$ nor adjacent to an element have total volume $\Omega(1/N^m)$, which we keep. The startpoints in the other intervals $T_i$ may then be thickened to a length $\Omega(1/N^{m/k})$ portion while still avoiding solutions. This gives a set with full Minkowski dimension and Hausdorff dimension $m/k$ avoiding solutions to $y = f(Tx)$. (I don't yet understand Minkowski dimension enough to understand this, but the techniques of the appendix make proving the Hausdorff dimension $1/k$ bound easy)

\section{Extension to Well Approximable Numbers}

If the coefficients of the linear transformation $T$ in the equation $y = f(Tx)$ are non-rational, then the images of startpoints under the action of $T$ do not form a lattice, and so points may not overlap so easily when avoiding solutions to the equations $y = f(Tx)$. However, if $T$ is `very close' to a family of rational coefficient linear transformations, then we can show the images of the startpoints are `very close' to a lattice, which will still enable us to find points avoiding solutions by replacing the direct combinatorial approach in the argument for integer matrices with a covering argument.

Suppose that $T$ is a real-coefficient linear transformation with the property that for each coefficient $x$ there are infinitely many rational numbers $p/q$ with $|x - p/q| \leq 1/q^\alpha$, for some fixed $\alpha$. For infinitely many $K$, we can therefore find a linear transformation $S$ with coefficients in $\mathbf{Z}/K$ with each coefficient of $T$ differing from the corresponding coefficient in $S$ by at most $1/K^\alpha$. Then for each $x$, we find
%
\[ \| (T - S)(x) \|_\infty \leq (n/K^\alpha) \| x \|_\infty \]
%
If we now consider $T_0, \dots, T_n$, splitting $T_1, \dots, T_n$ into length $1/N$ intervals, and considering $\mathbf{A}$ as in the last section, then $S(\mathbf{A})$ lie in a $k$ dimensional sublattice of $(\mathbf{Z}/KN)^m$, hence containing at most $(2A)^k (KN)^k = O_{T,n}((KN)^k)$ points. By our error term calculation of $T-S$, the elements of $T(\mathbf{A})$ are contained in cubes centered at these lattice points with side-lengths $2n/K^\alpha$, or balls centered at these points with radius $n^{3/2}/K^\alpha$. If $\| \nabla f \| \leq B$, then the images of the radius $n^{3/2}/K^\alpha$ balls under the action of $f$ are contained in length $Bn^{3/2}/K^\alpha$ intervals. Thus the total length of the image of all these balls under $f$ is $(Bn^{3/2}/K^\alpha)(2A)^k(KN)^k = (2A)^k Bn^{3/2} K^{k-\alpha} N^k$. If $k < \alpha$, then we can take $K$ arbitrarily large, so that there exists intervals with $\text{dist}(I,\mathbf{B}) = \Omega_{A,k,M}(1/N^k)$. But I believe that, after adding the explicit constants in, we cannot let $k = \alpha$.

\begin{remark}
    One problem is that, if $T$ has rank $k$, we might not be able to choose $S$ to be rank $k$ as well. Is this a problem? If $T$ has full rank, then the set of all such matrices is open so if $T$ and $S$ are close enough, $S$ also has rank $k$, but this need not be true if $T$ does not have full rank.
\end{remark}

\begin{example}
    If $T$ has rank 1, then Dirichlet's theorem says that every irrational number $x$ can be approximated by infinitely many $p/q$ with $|x - p/q| < 1/q^2$, so every real-valued rank 1 linear transformation can be avoided with a dimension one bound.
\end{example}

\section{Applications of Low Rank Coordinate Changes}

\begin{example}
Our initial exploration of low rank coordinate changes was inspired by trying to find solutions to the equation
%
\[ y - x = (u - w)^2 \]
%
Our algorithm gives a Hausdorff dimension $1/2$ set avoiding solutions to this equation. This equals Math\'{e}'s result. But this dimension for us now depends on the shifts involved in the equation, not on the exponent, so we can actually avoid solutions to the equation
%
\[ y - x = (u - w)^n \]
%
for any $n$, in a set of Hausdorff dimension $1/2$. More generally, if $X$ is a set, then given a smooth function $f$ of $n$ variables, we can find a set $X$ of Hausdorff dimension $1/n$ such that there is no $x \in X$, and $y_1, \dots, y_n \in X - X$ such that $x = f(y_1, \dots, y_n)$. This is better than the $1/2n$ bound that is obtained by Malabika and Fraser's result.
\end{example}

\begin{example}
For any fixed $m$, we can find a set $X \subset \mathbf{R}^n$ of full Hausdorff dimension which contains no solutions to
%
\[ a_1x_1 + \dots + a_nx_n = 0 \]
%
for {\it any} rational numbers $a_n$ which are not all zero. Since Malabika/Fraser's technique's solutions are bounded by the number of variables, they cannot let $n \to \infty$ to obtain a linearly independant set over the rational numbers. But since the Hausdorff dimension of our sets now only depends on the rank of $T$, rather than the total number of variables in $T$, we can let $n \to \infty$ to obtain full sets linearly independant over the rationals. More generally, for any Lipschitz continuous function $f: \mathbf{R} \to \mathbf{R}$, we can find a full Hausdorff dimensional set such that there are no solutions
%
\[ f(a_1x_1 + \dots + a_nx_n, y) \]
%
for any $n$, and for any rational numbers $a_n$ that are not all zero.
\end{example}

\begin{example}
The easiest applications of the low rank coordinate change method are probably involving configuration problems involving pairwise distances between $m$ points in $\mathbf{R}^n$, where $m \ll n$, since this can best take advantage of our rank condition. Perhaps one way to encompass this is to avoid $m$ vertex polyhedra in $n$ dimensional space, where $m \ll n$. In order to distinguish this problem from something that can be solved from Math\'{e}'s approach, we can probably find a high dimensional set avoiding $m$ vertex polyhedra on a parameterized $n$ dimensional manifold, where $m \ll n$. There is a result in projective geometry which says that every projectively invariant property of $m$ points in $\mathbf{RP}^d$ is expressible as a function in the ${m \choose d}$ bracket polynomials with respect to these $m$ points. In particular, our result says that we can avoid a countable collection of such invariants in a dimension $1/{m \choose d}$ set. This is a better choice of coordinates than Euclidean coordinates if ${m \choose d} \leq m$. Update: I don't think this is ever the case.
\end{example}

\begin{remark}
    Because of how we construct our set $X$, we can find a dimension $1/k$ set avoiding solutions to $y = f(Tx)$ for {\it all} rank $k$ rational matrices $T$, without losing any Hausdorff dimension. Maybe this will help us avoid solutions to more general problems?
\end{remark}

\begin{example}
Given a smooth curve $\Gamma$ in $\mathbf{R}^n$, can we find a subset $E$ with high Hausdorff dimension avoiding isoceles triangles. That is, if the curve is parameterized by $\gamma: [0,1] \to \mathbf{R}^n$, can we find $E \subset [0,1]$ such that for any $t_1, t_2, t_3$, $\gamma(t_1)$, $\gamma(t_2)$, and $\gamma(t_3)$ do not form the vertices of an isoceles triangle. This is, in a sense, a non-linear generalization of sets avoiding arithmetic progressions, since if $\Gamma$ is a line, an isoceles triangle is given by arithmetic progressions. Assuming our curve is simple, we must avoid zeroes of the function
%
\[ |\gamma(t_1) - \gamma(t_2)|^2 = |\gamma(t_2) - \gamma(t_3)|^2 \]
%
If we take a sufficiently small segment of this curve, and we assume the curve has non-zero curvature on this curve, we can assume that $t_1 < t_2 < t_3$ in our dissection method.

If the coordinates of $\gamma$ are given by polynomials with maximum degree $d$, then the equation
%
\[ |\gamma(t_1) - \gamma(t_2)|^2 - |\gamma(t_2) - \gamma(t_3)|^2 \]
%
is a polynomial of degree $2d$, and so Math\'{e}'s result gives a set of dimension $1/2d$ avoiding isoceles triangles. In the case where $\Gamma$ is a line, then the function $f(t_1,t_2,t_3) = \gamma(t_1) + \gamma(t_3) - 2\gamma(t_2)$ avoids arithmetic progresions, and Math\'{e}'s result gives a dimension one set avoiding such progressions. Rob and Malabika's algorithm easily gives a set with dimension $1/2$ for any curve $\Gamma$. Our algorithm doesn't seem to be able to do much better here.
\end{example}

\begin{example}
    What is the largest dimension of a set in Euclidean space such that for any value $\lambda$, there is at most one pair of points $x,y$ in the set such that $|x - y| = \lambda$.
\end{example}

\begin{example}
    What is the largest dimension of a set which avoids certain angles, i.e. for which a triplet $x,y,z$ avoids certain planar configurations.
\end{example}

\begin{example}
    A set of points $x_0, \dots, x_d \in \mathbf{R}^d$ lie in a hyperplane if and only if the determinant formed by the vectors $x_n - x_0$, for $n \in \{ 1, \dots, d \}$, is zero. This is a degree $d$ polynomial, hence Math\'{e}'s result gives a dimension one set with no set of $d+1$ points lying in a hyperplane. On the other hand, a theorem of Mattila shows that every analytic set $E$ with dimension exceeding one contains $d + 1$ points in a hyperplane. Can we generalize this to a more general example avoiding points on a rotational, translation invariant family of manifolds using our results?
\end{example}

\begin{example}
    Given a set $F$ not containing the origin, what is the largest Hausdorff dimension of a set $E$ such that for any for any distinct rational $a_1, \dots, a_N$, the sum $a_1E + \dots + a_NE$ does not contain any elements of $F$. Thus the vector space over the rationals generated by $E$ does not contain any elements of $F$. We can also take the non-linear values $f(a_1E + \dots + a_NE)$ avoiding elements of $F$. $F$ must have non-empty interior for the problem to be interesting. Then can we find a smooth function $f$ with non-nanishing derivative which vanishes over $F$, or a family of smooth functions with non-vanishing derivative around $F$.
\end{example}

\endinput

==> squarefree.tex <==
%% The following is a directive for TeXShop to indicate the main file
%%!TEX root = diss.tex

%\chapter{Constructing Squarefree Sets}
%\label{ch:Squarefree}

\endinput
